FieldFuzz: In Situ Blackbox Fuzzing of Proprietary Industrial Automation Runtimes via the Network

Networked Programmable Logic Controllers (PLCs) are proprietary industrial devices utilized in critical infrastructure that execute control logic applications in complex proprietary runtime environments that provide standardized access to the hardware resources in the PLC. These control applications are programmed in domain-specific IEC 61131-3 languages, compiled into a proprietary binary format, and process data provided via industrial protocols. Control applications present an attack surface threatened by manipulated traffic. For example, remote code injection in a control application would directly allow to take over the PLC, threatening physical process damage and the safety of human operators. However, assessing the security of control applications is challenging due to domain-specific challenges and the limited availability of suitable methods. Network-based fuzzing is often the only way to test such devices but is inefficient without guidance from execution tracing. This work presents the FieldFuzz framework that analyzes the security risks posed by the Codesys runtime (used by over 400 devices from 80 industrial PLC vendors). FieldFuzz leverages efficient network-based fuzzing based on three main contributions: i) reverse-engineering enabled remote control of control applications and runtime components, ii) automated command discovery and status code extraction via network traffic and iii) a monitoring setup to allow on-system tracing and coverage computation. We use FieldFuzz to run fuzzing campaigns, which uncover multiple vulnerabilities, leading to three reported CVE IDs. To study the cross-platform applicability of FieldFuzz, we reproduce the findings on a diverse set of Industrial Control System (ICS) devices, showing a significant improvement over the state-of-the-art.

==> Code/cmpdevice_log.tex <==
\begin{listing}[t]
\caption{NodeNameUnicode truncation}
\label{code:cmpdevice_log}
\begin{minted}[fontsize=\footnotesize, linenos, breaklines]{c}
Cmp=CmpNameServiceServer, Class=2, Error=0, Info=2, pszInfo=!!!! Node name was truncated. Original length: <len>86</len> characters
\end{minted}
\end{listing}

==> Code/cmpdevice_unicode.tex <==
\begin{listing}[t]
\caption{\texttt{NodeNameUnicode} bytestring}
\label{code:cmpdevice_unicode}
\begin{minted}[fontsize=\footnotesize, linenos, breaklines]{c}
[SysTarget] 
TargetVersionMask=0 
NodeNameUnicode=<bytestring>
\end{minted}
\end{listing}

==> Code/cmpmonitor2_entry.tex <==
\noindent\begin{minipage}{\columnwidth}





\begin{lstlisting}[caption={Pseudocode for CmpMonitor2\_\_Entry.}, label={code:cmpmonitor2_entry}, basicstyle=\footnotesize, language=C, frame=single]
int STATUS CmpMonitor2__Entry(INIT_STRUCT *init)
{
    init->CmpId = 50;
    init->ExportFunctions = CmpMonitor2_Export;
    init->ImportFunctions = CmpMonitor2_Import;
    init->GetVersion = CmpMonitor2_CmpGetVersion;
    init->HookFunction = CmpMonitor2_Hook;
    init->CreateInstance = CmpMonitor2_Create;
    init->DeleteInstance = CmpMonitor2_Delete;
    [..]
    return 0;
}
\end{lstlisting}


\end{minipage}

==> Code/disable_sysexcept.tex <==
\begin{listing}[t]
\caption{Disabling the internal exception handler}
\label{code:disable_sysexcept}
\begin{minted}[fontsize=\footnotesize, linenos, breaklines]{c}

[SysExcept]
Linux.DisableFpuInvalidOperationException=0
EnableFirstLevelHandling=0

\end{minted}
\end{listing}

==> Code/logger_cfg.tex <==
\begin{listing}[t]
\caption{Logger configuration}
\label{code:logger_cfg}
\begin{minted}[fontsize=\footnotesize, linenos, breaklines]{c}

[CmpLog]
Logger.0.Name=Plclog
Logger.0.Enable=1
Logger.0.Backend.0.ClassId=0x0000010B
Logger.0.Backend.1.ClassId=0x00000104
Logger.0.Filter=0xFFFFFFFF
CmpApp.Filter=0xFFFFFFFF
CmpChannelMgr.Filter=0xFFFFFFFF
CmpChannelServer.Filter=0xFFFFFFFF

\end{minted}
\end{listing}

==> Code/main_packed.tex <==
\begin{listing}[t]
\caption{Pseudocode for main function.}
\label{code:main_function}
\begin{minted}[fontsize=\footnotesize, highlightlines={9, 10}, highlightcolor=yellow, linenos, breaklines]{c}
__int64 __fastcall main(int a1, char **a2, char **a3)
{
    size_t v3;

    dword_8A4AED0 = a1;
    qword_8A4AEC8 = (__int64)a2;
    dl_iterate_phdr(callback, 0LL);
    v3 = len;
    mprotect(addr, len, 7);
    sub_85568C0(qword_82C83C0, v3);
    return 0;
}
\end{minted}
\end{listing}

==> Code/stateful_cve.tex <==
\begin{listing}[t]
\caption{\texttt{CmpTraceMgr} commands in sequence.}
\label{code:stateful_cmptracemgr}
\begin{minted}[fontsize=\footnotesize, linenos, breaklines]{c}
Packet ReadList
Packet create
Add records 
Complete packet
Start trace
Set trigger
Variables are recorded
Stop
Packet restart / start / delete
\end{minted}
\end{listing}

==> Tables/codesyscve.tex <==
\begin{table}[t]
\caption{Increasing number of Codesys CVEs~\cite{misc:codesys-cve}.}
\label{table:codesys_cve}
\resizebox{\columnwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Year}    & \textbf{2011} & \textbf{2012} & \textbf{2013} & \textbf{2014} & \textbf{2015} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021}& \textbf{2022}  \\ \hline
\textbf{\# CVEs} & 4             & 7             & 1             & 3             & 3             & 2             & 6             & 14            & 5             & 35  & 24           \\ \hline
\end{tabular}}
\end{table}

==> Tables/errorcodes.tex <==
\begin{table}[!htbp]
\centering
\caption{The status codes used by FieldFuzz to uncover system states.}
\label{table:error_codes}
\resizebox{\columnwidth}{!}{\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Error} & \textbf{ID} & \textbf{Error} & \textbf{ID} \\ \hline
Ok & 0x00 & VersionMismatch & 0x1F \\ \hline
Failed & 0x01 & TypeMismatch & 0x20 \\ \hline
Parameter & 0x02 & IdMismatch & 0x21 \\ \hline
NotInitialized & 0x03 & OperationDenied & 0x27 \\ \hline
Version & 0x04 & SecurityChecksFailed & 0x39 \\ \hline
Timeout & 0x05 & InvalidSequence & 0x3A \\ \hline
NoBuffer & 0x06 & TooManyRetries & 0x3D \\ \hline
Pending & 0x0A & AlignmentError & 0x3E \\ \hline
NumPending & 0x0B & PasswordChangeRequired & 0x3F \\ \hline
NotImplemented & 0x0C & Reauthenticate & 0x40 \\ \hline
InvalidId & 0x0D & Relogin & 0x41 \\ \hline
Overflow & 0x0E & NotReadyYet & 0x45 \\ \hline
BufferSize & 0x0F & ActivateUserMgt & 0x46 \\ \hline
NoObject & 0x10 & NoUserMgmt & 0x47 \\ \hline
NoMemory & 0x11 & NetFailed & 0x100 \\ \hline
Duplicate & 0x12 & NetNotConnected & 0x101 \\ \hline
MemoryOverwrite & 0x13 & NetMsgSize & 0x102 \\ \hline
InvalidHandle & 0x14 & NetNoRoute & 0x103 \\ \hline
EndOfObject & 0x15 & NetTimeout & 0x104 \\ \hline
NoChange & 0x16 & NetPkgInvalid & 0x105 \\ \hline
InvalidInterface & 0x17 & NetProtocolid & 0x106 \\ \hline
NotSupported & 0x18 & L7TagMissing & 0x300 \\ \hline
NoAccessRights & 0x19 & L7UnknownCmdGrp & 0x301 \\ \hline
OutOfLimits & 0x1A & L7UnknownCmd & 0x302 \\ \hline
EntriesRemaining & 0x1B & AppNotLoaded & 0x504 \\ \hline
InvalidSessionId & 0x1C & AppNoSessionId & 0x505 \\ \hline
Exception & 0x1D & AppBPBreakpointNotSet & 0x50E \\ \hline
SignatureMismatch & 0x1E &  &  \\ \hline
\end{tabular}}
\end{table}

==> Tables/test.tex <==
\appendix
Hello world

==> Text/CodesysStack.tex <==
% \section{Appendix}
% \label{app:a}
% \subsection{FRD Exploit Development Capabilities}

% The FRD is also an essential tool for crash analysis, aiding exploit development. Specifically, it provides the following capabilities to the security analyst:

% \noindent \textbf{Interaction with each layer}.
% During the exploit debugging, it is common for some packets to cause errors which prevent them from entirely being processed by the runtime network stack. As a result, such packets fail to reach the service layer and are rejected by the Channel Server or Router for various reasons. To address this, the FRD allows investigating such cases by interacting with each layer and gradually testing the packet processing.

% \noindent \textbf{Wireshark dissector}.
% The full-featured dissector for Codesys v3 protocol enables the use of Wireshark with advanced filter expressions and custom columns for every aspect of the Codesys v3 stack. Based on the gained knowledge in this work, we provide it with symbols to translate the packet data into human-readable components, command, and field names. Despite the implementation in Lua, the resulting performance is adequate for handling live capture sessions between {\FRAMEWORKNAME} and the target device for long periods. 
% The dissector significantly streamlines the process of input corpus collection, crash investigation, and exploit development.

% \noindent \textbf{Binary tag encoder}.
% An interactive binary tag encoder of the FRD allows to conveniently parse and craft the binary tag payloads and display them in a readable form.
% It is used in conjunction with the Wireshark dissector, which pastes values from a packet field to the encoder. The latter allows its recursive printing, modification, and re-encoding in place.

% \noindent \textbf{Exploit generation}.
% FRD provides multiple single-file standalone exploit templates which embed the compact implementation of a communication routine. These are minimal features required to establish a connection and send a payload to the components. 
% We use these to generate standalone proof-of-concept exploits for the crashes found in Section \ref{sec:results} that do not require the FRD.

% \noindent \textbf{Remote memory dumps}.
% A handy feature of the FRD is obtaining the hexdumps of the PLC memory regions via the network.
% This is implemented by requesting \texttt{CmpApp} (GetAreaAddress) and \texttt{CmpPlcShell} (Execute \texttt{0x1}).
% To avoid reply fragmentation while retrieving a long hexdump, FRD splits the requested address range and instead requests 128-byte chunks.

% \noindent \textbf{Retrieving runtime logs}.
% Specific components of the runtime use a standard logger to append messages grouped into categories through an exported interface which is part of \texttt{CmpLog}.
% The default behavior of the runtime is to rotate the log buffer in a dedicated region of the controller memory. The FRD can request logs from this buffer by implementing \texttt{LoggerList} \texttt{0x03} and \texttt{GetEntries} \texttt{0x01} commands of \texttt{CmpLog}, to scan for exceptions, observe events and errors, or query invariant runtime fields such as application name logged by \texttt{CmpApp}.
% \vspace{-0.3cm}
%\subsection{Additional fuzzing campaigns}

%\subsubsection{Fuzzing CmpDevice Component (CVE-2022-22508)}









% \clearpage
% \section{Scratchpad}

% This section discusses the development of the Codesys v3 communication protocol dissector for Wireshark, written in Lua. We start by analyzing the runtime for Linux x64 to understand memory segments and their components by reverse engineering. Finally, we understand the Codesys v3 protocol network stack to determine the essential components involved in network communication, payload format, and parsing.

% % A 29-09-21: later need to double-check "packed-unpacked" info, num of functions against binaries

% \noindent \textbf{Learning from device description files.} These are huge XML files, appropriately named \texttt{codesyscontrol.devdesc} (more than 3000 lines of text for Beaglebone Black) that ship with the corresponding target enlisting the hardware capabilities of the device using a structured format. The IDE explicitly imports these devdesc files before connecting to the target PLC. We use it for identifying attributes regarding the device in the \texttt{<Device>} tag checked for consistency during the connection, driver information, task configuration information, memory layout of the controller, capabilities, and other general knowledge of the platform. 

% \noindent \textbf{Understanding memory segments.} Runtime separates data and IEC (code) into separate memory segments, observable in the devdesc file, which contains the number of areas and their corresponding types. Typically, data is in area0 with the type flag of \texttt{0xFE9F} and code section in area3 with type flag of \texttt{0x0040}.

% % \noindent \textbf{Frequently observed functions.}
% % A 28-09-21: Reversing (renaming) of TOP 20 most frequently called functions helped to find logging, component init, events, binary tag reader-writer commands. We can specify a table of those ida top 20 funcs and their meaning %

% % \noindent \textbf{Monitoring bytecode interpreter}
% %A 29-09-21: Deeper overview of the Monitor2 bytecode %interpreter, opcodes, stack guard, hardcoded canary can be %provided later
% % Table of 57 opcodes and their meaning
% % Implemented python disassembler explained




% % CMRegisterAPI


% % use the dissector and show packet info
% % Worth noting somewhere that every TCP packet with payload is handled by ~12 functions of the network stack before it can reach the target component


% \subsection{Implementing the Dissector}

% %\noindent \textbf{Implementing the dissector.} From the knowledge acquired by reversing the runtime for Linux x64, we implement a corresponding Wireshark dissector in Lua. During the implementation, we had to take care of authentication because, with the default configuration of the runtime, there is a need for authenticating in at least two layers for properly sending the commands to the components: the device login stage and the application login stage. Upon successful completion of the login, the \texttt{CmpDevice}, and \texttt{CmpApp} generate session sequence Id, which is validated in all the subsequent requests. {\FRAMEWORKNAME} maintains the session information to establish a stateful fuzzing session with the runtime. Furthermore, another complication for the dissector and client library is the custom fragmentation of payloads, independent of the TCP layer, handled by the current implementation of {\FRAMEWORKNAME}.\\

% Using the acquired knowledge, we implement the Codesys v3 communication protocol dissector. During the implementation, we had to take care of authentication because, with the default configuration of the runtime, there is a need for authenticating in at least two layers for properly sending the commands to the components: the device login stage and the application login stage. Upon successful completion of the login, the \texttt{CmpDevice}, and \texttt{CmpApp} generate session sequence ID, which is validated in all the subsequent requests. {\FRAMEWORKNAME} maintains the session information to establish a stateful fuzzing session with the runtime. Furthermore, another complication for the dissector and client library is the custom fragmentation of payloads, independent of the TCP layer, handled by the current implementation of {\FRAMEWORKNAME}.

% \noindent \textbf{Correlation with IDE commands.} Empowered with the ability to dissect the network layers and understand the payload layout, we record the traffic between the Codesys Development System and the Codesys Gateway service forwarded to the PLC. By issuing IDE commands, we could correlate the actions executed from its GUI to service groups and command codes, thus understanding the responsibility of corresponding components. Some important commands corresponding to the components at the service layer are presented in Table~\ref{table:commands}.
   
% % The command (action) consists of: CMP_ID (Service Group ID) + CMD_ID + payload (binary tags)    %

% % Introduction to find how to find a component in the reverse enng database
% % Maybe some block diagram / fictional component (opensource component)



% \subsection{Codesys Network Stack}\label{subsec:network_stack}
% The runtime utilizes a proprietary stack of protocols that we will refer to as the Codesys v3 protocol to facilitate network communication between Codesys network nodes, including the development system and the runtime. Security researchers at Kaspersky examined a variant of the runtime ported for Raspberry Pi, and its TCP network communication. It should be noted that the details of the Codesys v3 network stack are the contribution of~\cite{misc:kaspersky_codesys}. On the other hand, in this work, we reverse engineer the runtime binary and its communication deeper to uncover and understand the internals of the components utilized by the runtime for controlling the execution of the control application. Moreover, we use the extracted knowledge to propose a stateful fuzzing methodology for the control application and the runtime components that are reachable from the network.

% The Codesys v3 network stack consists mainly of four different layers: Block Driver, Datagram, Channel, and Service Layer. Each layer operates independently from the other. Each layer has components specific to it for processing incoming packets. Typically, each packet is processed by more than 12 component functions before reaching its destination service.

% \begin{figure}[t]
% \centering
% \includegraphics[clip, trim=4.2cm 1.8cm 4.8cm 5cm, width=\columnwidth]{Diagram/Packet.pdf}
% \caption{Important fields at different layers of the Codesys v3 Protocol.}
% \label{fig:network_stack}
% \end{figure}

% \noindent \textbf{Block driver layer.} The components at this layer are responsible for facilitating communication over the physical interfaces. Here, the component \texttt{CmpBlkDrvTcp} is of our interest, which implements the communication over TCP via Ethernet, in this case using the socket managed by the underlying OS. It adds two additional fields with each message,~\blockParam{1} a \textit{magic} number to be verified and~\blockParam{2} the total number of bytes in the packet: \textit{length} as shown in Fig.~\ref{fig:network_stack}. Next, \texttt{CmpBlkDrvTcp} transfers the rest of the packet to \texttt{CmpRouter} component of the Datagram layer.

% \noindent \textbf{Datagram layer.} \texttt{CmpRouter} is the most interesting component at this layer, which is responsible for detecting Codesys nodes in the network and routing packets. The received data is passed as an argument to its \texttt{RouterHandleData} function which parses the following fields:~\datagramParam{1} One byte \textit{magic} number (\texttt{0xc5}) inserted by \texttt{CmpRouter}.~\datagramParam{2} \textit{hop\_info} bit structure, which consists of 5-bit \textit{hop\_count} and 3-bit \textit{header\_length}. Similar to hop count in regular packets, each Codesys network node upon receiving the Codesys v3 protocol packet over network, decrements the \textit{hop\_count} before transmitting it to the next network node. \textit{header\_length} indicates the number of bytes to the next data size field.~\datagramParam{3} Next are the packet settings: \textit{packet\_info} of which the first two bits indicate \textit{priority} (0: low, 1: normal, 2: high, 3: emergency) of the processed packet. Next is the \textit{signal} bit used by \texttt{CmpRouter} to indicate error. The \textit{type\_address} specifies the type of transmitted address (0: full address, 1: relative address) and the last field is \textit{length\_data\_block} specifying the maximum data size accepted by the recipient.~\datagramParam{4} Next, the \textit{service\_id} identifies the destination service. A service ID of 1 and 2 is used for request and response, respectively, by the address service for detecting the live network nodes. A value of 3 for request and 4 for response to the name service, utilized for receiving information about a node. Finally, a value of 64 (\texttt{0x40}) for both requesting and responding to the channel service to query the server and the communication channel manager.~\datagramParam{5} The \textit{message\_id} field is filled by the sender (generally the current time) to identify the message uniquely.~\datagramParam{6} Next is the \textit{lengths} field in which twice the value of the length in the most significant 4 bits corresponds to the size of the receiver field and is similar for the least significant 4 bits for the sender.~\datagramParam{7} The address of the \textit{sender} of the message and its \textit{receiver}, and finally the optional \textit{padding}.

% Fig.~\ref{fig:network_stack} shows the fields processed by the datagram layer. When the value of the \textit{service\_id} is 1, 2, 3 or 4, the packet is processed by \textit{CmpRouter}, however, when the ID is 64 (\texttt{0x40}), the packet is forwarded to the \texttt{CmpChannelManager} component in the channel layer.

% \noindent \textbf{Channel layer.} This is the next layer in the Codesys PDU stack responsible for ensuring synchronized communication, verifying the integrity of transmitted data, acknowledging the delivery, and transmitting a large amount of data. \texttt{CmpChannelMgr} is the main component of the layer handling the tasks mentioned above. It creates a buffer for messages, opening, and closing of communication channels, information delivery, and more. \texttt{CmpChannelClient} is the client of the channel to handle requests and process responses from the channel server. Fig.~\ref{fig:network_stack} shows the important fields for the corresponding packet type, also mentioned here:~\channelParam{1} This layer specifies certain commands (\textit{command\_id}) for the communication channel manager. A dedicated Layer 3 channel has to be open, kept alive, and closed for successful communication. The \textit{command\_id} of \texttt{0x1} (BLK) indicates the transfer of data to the next layer, \texttt{0x2} (ACK) is the receipt for data communication, and \texttt{0x3} (KEEPALIVE) for keeping the channel active. The BLK packet type is of interest to us for controlling fuzzing inputs to the IEC application binary.~\channelParam{2} \textit{flag} field with a value of \texttt{0x81} indicates that the data is the first of its transmission. However, if the least significant bit is not set, the message continues the previous message.~\channelParam{3} The \textit{channel\_id} for identifying the open channel.~\channelParam{4} \textit{blk\_id} is the ID of the current BLK message which is incremeneted by the sender.~\channelParam{5} \textit{ack\_id} is the ID of the previous ACK message.~\channelParam{6} The \textit{remaining\_data\_size} field is the size of the expected data remaining in the packet.~\channelParam{7} Finally, the \textit{checksum} field with the CRC32 checksum for the remaining data.

% After the \texttt{CmpChannelMgr} finishes processing, the remaining data passes to the service layer for final processing.

% \noindent \textbf{Services layer.} This layer, as shown in Fig.~\ref{fig:network_stack} is responsible for querying the requested service while transmitting the operating settings. The message header consists of:~\serviceParam{1} \textit{protocol\_id} indicating the protocol handle for utilization to pass the data over to the relevant service. It supports \texttt{HeaderTagProtocol} with an ID value of \texttt{0xCD55}, indicating that the \textit{protocol\_data} field consists of tags. The request, command payloads, and replies from the service layer of the runtime are delivered inside nested binary structures, called tags. Each tag starts with its ID, which often corresponds to the payload or status code, the length, and the data. We implement a recursive encoder to work with the requests and responses at this level. It also supports \texttt{SecureProtocol} with an ID value of \texttt{0x7557} allowing secure data transfer needing decryption before processing.~\serviceParam{2} \textit{header\_size} is the size of the \textit{protocol\_header} and does not contain the size of the current and previous fields.~\serviceParam{3} \textit{service\_group} refers to the ID of the queried service. Runtime has a unique ID for each available service and identifies the corresponding component for processing the service request. The layer sets the most significant bit of the ID in the response message.~\serviceParam{4} \textit{service\_id} refers to the commands available for a specific service. For example, Table~\ref{table:components} mentions some of the critical components/services with their corresponding IDs.~\serviceParam{5} Then \textit{session\_id} identifying the session, \textit{content\_size}, \textit{additional\_data}, and \textit{protocol\_data} for size of the data, additional data and the data generated for the utilized protocol.

% \noindent \textbf{Tags.} It is the interface to provide service settings to the runtime components. Each tag starts with its ID:~\tagsParam{1} \textit{tag\_id}, which often corresponds to type of payload or status code, the \textit{tag\_size} and the \textit{tag\_data} and some \textit{additional\_data}. Fig.~\ref{fig:network_stack} shows the tag fields for writing to a variable.~\tagsParam{2} \textit{data\_size} is the size of the data to be written,~\tagsParam{3} \textit{write\_value} is the value to be written and~\tagsParam{4} \textit{write\_offset} is the offset of the variable from the start of the data section (area 0).


% \section{Codesys components}


% Some of the critical runtime components are:

% \noindent \textbf{Component manager.} The Component Manager (CM) is responsible for launching and initializing all other components. The runtime uses a ``.cfg" configuration file to store the keys and parameters for configuring components. A dedicated component \texttt{CmpSettings} registers an API, and other components then utilize that to acquire parameters from the configuration file.

% \noindent \textbf{System components.} These components can be platform-specific and are responsible for interaction with the hardware and the underlying OS. This includes memory management tasks, communication with sockets and physical ports, file system, and more.
% While most of components in other groups are normally generic and are developed by Codesys itself, the System Components usually have to be adapted by the device vendor.

% \noindent \textbf{Communication components.} This is the collection of components responsible for communicating with external entities over the network. It implements the Codesys v3 protocol stack to enable routing and communication in an industrial network with mixed segments of Ethernet, CAN, Serial, Sercos and other mediums.

% \noindent \textbf{Application components.} These are required for controlling the execution of the PLC program and other operations.

% \noindent \textbf{Core components.} The components are employed to control logging, event signals and other key operations of the PLC~\cite{misc:kaspersky_codesys}.


% \subsection{Important Runtime Components}
% In this section, we discuss some components pertinent to the functioning of {\FRAMEWORKNAME}.

% \noindent \textbf{CmpDevice.} To establish connection with the runtime, Codesys requires authentication at the device level using~\texttt{DeviceServiceHandler} function in \texttt{CmpDevice}. It provides functionalities such as device login (\texttt{0x02}), logout (\texttt{0x03}), checking the established channel (\texttt{0x07}) and more.

% \noindent \textbf{CmpPlcShell.} This is the terminal controller built into the runtime, allowing some primitive control over the execution of the application. It implements commands such as \texttt{startprg}, \texttt{stopprg} to start and stop the execution of the application, \texttt{applist} to retrieve the list of active applications, \texttt{getprgstat} to get the state of the application, and finally \texttt{resetprg}, \texttt{resetprgcold} to reset all the variables and the program.

% \noindent \textbf{CmpApp.} This component enables fine-grained control over the execution of the application. It allows login (\texttt{0x01}) and logout (\texttt{0x02}) from the application, start (\texttt{0x10}), stop (\texttt{0x11}), reset (\texttt{0x12}) execution of the application. Furthermore, it provides other supplementary functionalities to set (\texttt{0x13}) and delete (\texttt{0x15}) breakpoint, allows single cycle execution (\texttt{0x22}), and more. \texttt{CmpApp} provides better control over the execution of the application with even support for single cycle execution, and is therefore our choice for controlling the execution of the application in {\FRAMEWORKNAME}.

% \noindent \textbf{CmpMonitor2.} This component is critical for providing fuzzing inputs to the IEC application on the fly. It provides the read (\texttt{0x01}) and write (\texttt{0x02}) for the input variable. It also needs the offset of the variable in area 0, the data section of the runtime, to write to the corresponding memory location.

% Some other components are: \texttt{CmpSettings}, which enables reading and editing the runtime settings. \texttt{CmpIecTask} handles IEC tasks such as creating, deleting, collecting monitoring information for the application manager. \texttt{CmpBinTagUtil} implements function to read and write data for BinTag format. \texttt{CmpMgr} for loading and unloading components dynamically. \texttt{CmpBlkDrvTcp}, \texttt{CmpChannelMgr}, \texttt{CmpRouter} and \texttt{CmpSrv} are essential components for routing the Codesys v3 network packet to the appropriate requested service of the runtime. \texttt{SysExcept} handles all the exceptions available across the runtime, whereas, \texttt{CmpCoreDump} is used to dump the memory allowing crash investigations. CmpIecVarAccess allows symbolic access to variables,  \texttt{CmpOPCUAProviderIecVarAccess}, and \texttt{ModbusTcpClient} for reading/writing variable values using OPC UA protocol and Modbus respectively.


==> Text/Methodology.tex <==
% Emphasize that it is system fuzzing



%The bare-metal IO is often seen in literature as primary communication method for PLC \cite{usenix21icsfuzz} \cite{Garcia2017Jan}. However, with variety of industrial protocols being wrapped into TCP and due to limitations of I/O slots capacity and voltage range, the barematal IO is often not engaged in plant operation. The plant in this case can be operated by Ethernet.
%The input supply to the control variables through fieldbuses requires explicit declaration of such exports in the control project.
%The component also has a corresponding library which can be called from IEC application. For this reason, some documentation is available on its interface \cite{help_cmpvaraccess}.

%\noindent \textbf{Input supply.} %In literature, often bare-metal IO is utilized as the primary communication method for PLCs~\cite{proc:icsfuzz, art:malware_physics}. However, such an approach is not scalable and is often specific to the model of the PLC. Another approach is to utilize the Modbus protocol from the Fieldbus family of network communication protocols. Our initial implementation of the input manipulator, based on ModbusTcpClient~\cite{misc:pymodbus} successfully fed inputs to the Codesys program during runtime. Nevertheless, such an approach requires the project to include the Modbus slave object to receive read and write commands, requiring explicit declarations of such exports in the control project, not enabled by default. Generally, HMI display and modify the inputs to a program using OPC UA; however, for Codesys, this is not compiled into all distributions, requires a license verified by \texttt{CmpOPCUAProviderIecVarAccess} otherwise, it shuts down the OPC UA server in 2 hours. Generally global variable list or its part are mapped in the project to Symbol Configuration to enable variable access by name by utilizing \texttt{CmpIecVarAccess}~\cite{misc:help_cmpvaraccess}. Furthermore, when declaring symbolic variables for the project, the IDE provides an option to enable ``Direct IO access" for symbolic configuration. In this way, using CmpIecVarAccess, IO memory segments can be accessed remotely. However, the approaches mentioned above require explicit modifications to the configuration of the control project for supporting certain Fieldbus protocols or export variables. {\FRAMEWORKNAME} utilizes a universal approach without requiring modifications to the project settings enabling read and write to any variable regardless of the project properties. It uses the \texttt{CmpMonitor} and \texttt{CmpMonitor2} components to ensure the fastest way to read and write arbitrary variables from their respective memory segments.

% \noindent \textbf{Input supply.} {\FRAMEWORKNAME} is a black-box approach to fuzzing the control runtime and the IEC applications. Since the IEC application runs in the context of the control runtime, it is not easy to obtain meaningful feedback from the currently executing control program. So, the current implementation of {\FRAMEWORKNAME} utilizes random inputs and lacks input mutation based on fuzzing feedback.

%\noindent \textbf{Crash monitoring.} {\FRAMEWORKNAME} surveys \texttt{CmpApp} and \texttt{CmpPlcShell} components over the network to retrieve the status of the execution of the control application binary. Upon exception, a core dump and crash logs from \texttt{CmpLog} are retrieved from the controller remotely for further investigation.

    
%\noindent \textbf{Code coverage.} Unlike ICSFuzz that performed the intrusive operation of overwriting the NOPs included in the compiled control application binary, {\FRAMEWORKNAME} leverages \texttt{CmpAppBP} to set breakpoints in the control program. We can then query \texttt{CmpApp} to retrieve the hit count of the set breakpoints and calculate the coverage statistics in real-time based on these observations.




==> Text/fieldfuzz.tex <==
% [Provide an overview/intution for fieldfuzz here. What are the main challenges that AFL/ICSFuzz was not able to solve? How are we planning to connect to the IEC applications, and control them? Keep reversing details to a minimum. Provide high level design of FRD and Ghost parts here, to lead up to next section ]

% Proposal: We put challenges in Section III, and how we work around them in IV. 

Item list:
\begin{itemize}
    \item FF overview / intuition 
    \item High level FF + Ghost design overview [overlap with Section III-D]
    \item Challenges that AFL/ICSFuzz don't solve [Also in Section III-B]
    \item How we plan to connect to IEC applications and control them [overlap with Section III-D]
\end{itemize}
 
\begin{figure*}[t]
\centering
\includegraphics[clip, trim=0cm 6cm 0cm 0.48cm, width=\linewidth, keepaspectratio]{Diagram/System_Design.pdf}
\caption{{\FRAMEWORKNAME} methodology overview for fuzzing IEC applications and the control runtime.}
\label{fig:methodology}
\vspace{-0.3cm}
\end{figure*}


